Local form factor subtraction for three-loop QCD corrections to electroweak production in quark-antiquark annihilation

We extend a local subtraction framework to three-loop QCD corrections for the production of multiple electroweak bosons in quark-antiquark annihilation. We derive two-loop Ward identities that ensure the factorisation of most collinear singularities from the hard-scattering process in the sum over integrands. Infrared and ultraviolet singularities are removed point-by-point in loop momentum space using a minimal set of counterterms, which can be integrated analytically in terms of known master integrals. Additional counterterms eliminate non-factorising terms arising from loop momentum shifts and one-loop corrections to the gluon three-point function. We identify previously unknown non-factorising loop polarisation effects in the single-collinear regions, which pose challenges for local integrability and require further investigation. The techniques presented here are a first crucial step in formulating a systematic approach for constructing finite integrands for general electroweak amplitudes at three-loop order.

==> M1_finite.tex <==
\section{Review of the one-loop subtraction}
\label{sec:M1_fin}
In this section we review the regularisation of the one-loop amplitude for the quark-antiquark annihilation process. This will serve as the paradigmatic case before we move on to the more complicated three-loop amplitude. Many of the salient features of the \acs{ffs} method appear starting at two-loop order.  

We re-organise the one-loop integration according to the prescription in eqs.~\eqref{eq:Mfin_Msing} and~\eqref{eq:Mfin},
\begin{align}
{M}^{(1)} \equiv \int_l\,
\mathcal{M}^{(1)}_\text{finite}(l)
+\int_l\, 
{\mathcal M}_\text{\rm singular}^{(1)}(l)\,.
\label{eq:M1-IRUV-sub}
\end{align}
where ${\mathcal M}_\text{\rm singular}^{(1)}$ is the set of counterterms, local in loop-momentum space, that approximate the one-loop integrand in all its \acs{uv} and \acs{ir} divergent limits. Explicitly,
\begin{align}
    {\mathcal M}_\text{\rm singular}^{(1)}(l) =
    \mathcal{F}^{(1)}_\text{UV-finite}(l)[\mathbf{P}_1\,M^{(0)}\,\mathbf{P}_1] + \mathscr{R}_{l\to \infty}\,\mathcal{M}^{(1)}(l)\,,
\end{align}
with
\begin{align}
    \mathcal{F}^{(1)}_\text{UV-finite}(l)
    = (1-\mathscr{R}_{l\to \infty})\mathcal{F}^{(1)}(l)\,.
\end{align}
The one-loop form factor counterterm $\mathcal{F}^{(1)}(l)$ removes both soft ($l\sim 0$) and collinear ($l\,||\,p_1$ or $l\,||\,p_2$) singularities from the one-loop integrand $\mathcal{M}^{(1)}(l)$.


We emphasise that the finiteness of the term $\mathcal M_\text{finite}^{(1)}$ is achieved only by considering the sum over all one-loop diagrams.





==> app_UV_old.tex <==
\section{UV approximated two-loop subgraphs}
\label{app:uv_old}
In this appendix we provide the explicit single- and double-UV approximations for the vertex functions $V_i^{(2,X_1)\,\mu}$ and $W_i^{(2,X_2)}$ with $X_1\in\{UL,XL,3V\}$ and $X_2\in\{UL,XL,4V,d3V\}$ which were introduced in secs.~\ref{sec:QED_vertex_2L} and~\ref{sec:QCD_vertex_2L}. Together, they define the two-loop QCD corrections to the electroweak vertex 
and quark-antiquark-gluon vertex.
Additionally, we include the local UV approximations for the kinematic functions $S^{(2,UL)}$, $S^{(2,XL)}$ and $S^{(2,3V)}$, which define the two-loop QCD corrections to the quark-self energy $\Pi_{qq}^{(2)}$ introduced in sec.~\ref{sec:quark_self_energy_2L}.

\subsection{Single-UV region}
We begin with the single-\acs{uv} limits of the uncrossed ladder vertex functions, which take the form,
\begin{align}
    \begin{split}
        &V^{(2,UL)\,\mu}_{1\,\text{single-UV}}
        (p,q,k,l) 
        \\&\qquad\qquad=
        -\frac{\gamma^\alpha (\s{p} + \s{l} + \s{q}) S^{(1)}_\text{UV} (p+l+q,k)(\s{p} + \s{l} + \s{q}) \gamma^\mu (\s{p} + \s{l}) \gamma_\alpha}{l^2 (p+l)^2 ((p+l+q)^2)^2}\,,
        \label{eq:EW_vertex_2L_UL_V1_UV}
    \end{split}\\
        \begin{split}
        &V^{(2,UL)\,\mu}_{2\,\text{single-UV}}(p,q,k,l) =
        -\frac{\gamma^\alpha (\s{p} + \s{l} + \s{q}) \gamma^\mu (\s{p} + \s{l})  S^{(1)}_\text{UV} (p+l,k)(\s{p} + \s{l}) \gamma_\alpha}{l^2 ((p+l)^2)^2 (p+l+q)^2 }\,,
        \label{eq:EW_vertex_2L_UL_V2_UV}
    \end{split}\\
    \begin{split}
        &V^{(2,UL)\,\mu}_{3\,\text{single-UV}}(p,q,k,l) = 
        \frac{\gamma^\alpha (\s{p} + \s{l} + \s{q}) V^{(1)\,\mu}_\text{UV}(k)  (\s{p} + \s{l})  \gamma_\alpha}{l^2 (p+l)^2 (p+l+q)^2}\,.
        \label{eq:EW_vertex_2L_UL_V3_UV}
    \end{split}
\end{align}
Here, we have simply replaced the one-loop functions $V^{(1)\,\mu}$ and $S^{(1)}$ in eqs.~\eqref{eq:EW_vertex_2L_UL_V1} and~\eqref{eq:EW_vertex_2L_UL_V2} with their \acs{uv}-expansions, $V^{(1)\,\mu}_\text{UV}$ and $S^{(1)}_\text{UV}$ defined in eqs.~\eqref{eq:V_1L_UV} and~\eqref{eq:S_1L_UV}.
For the crossed ladder diagrams, it can be shown by simple power counting that the vertex function $V^{(2,XL)\,\mu}_{3}$ defined in eq.~\eqref{eq:EW_vertex_2L_XL_V3} is finite when either loop momentum becomes large. 
We have,
\begin{align}
\begin{split}
    V^{(2,XL)\,\mu}_{1\,\text{single-UV}}(p,q,k,l) &=
    \frac{V^{(1)\,\alpha}_\text{UV}(k)(\s{p} + \s{l} + \s{q}) \gamma^\mu  (\s{p} + \s{l}) \gamma_\alpha }{ l^2 (p+l)^2 (p+l+q)^2} \,,
    \label{eq:EW_vertex_2L_XL_V1_UV}
\end{split}\\
\begin{split}
     V^{(2,XL)\,\mu}_{2\,\text{single-UV}}(p,q,k,l) &=\frac{\gamma_\alpha (\s{p} + \s{l} + \s{q}) \gamma^\mu  (\s{p} + \s{l})V^{(1)\,\alpha}_\text{UV}(k)}{l^2 (p+l)^2(p+l+q)^2}\,,
     \label{eq:EW_vertex_2L_XL_V2_UV}
\end{split} \\
\begin{split}
     V^{(2,XL)\,\mu}_{3\,\text{single-UV}}(p,q,k,l) &=0\,.
     \label{eq:EW_vertex_2L_XL_V2_UV}
\end{split}
\end{align}
Likewise, for the three-gluon vertex graphs we obtain
\begin{align}
\begin{split}
    V^{(2,3V)\,\mu}_{1\,\text{single-UV}}(p,q,k,l) &=\frac{W^{(1)\,\alpha}_\text{UV}(k)(\s{p}+\s{l}+\s{q})\gamma^\mu(\s{p}+\s{l})\gamma_\alpha}{l^2(p+l)^2(p+l+q)^2}\,,
    \label{eq:EW_vertex_2L_3V_V1_UV}
    \end{split}\\
    \begin{split}
    V^{(2,3V)\,\mu}_{2\,\text{single-UV}}(p,q,k,l) &=\frac{\gamma_\alpha(\s{p}+\s{l}+\s{q})\gamma^\mu(\s{p}+\s{l})W^{(1)\,\alpha}_\text{UV}(k)}{l^2(p+l)^2(p+l+q)^2}\,.
    \label{eq:EW_vertex_2L_3V_V2_UV}
\end{split}
\end{align}
The colour coefficients multiplying the single-UV approximations in eqs.~\eqref{eq:EW_vertex_2L_UL_V1_UV}-\eqref{eq:EW_vertex_2L_3V_V2_UV} will depend on the flavour of the external particle.


==> pole_structure.tex <==
\subsection{Divergences to three-loop order}
Let us consider an on-shell $n$-point \ac{qcd} amplitude $\mathcal{M}$ containing $m$ external massless partons (quarks or gluons) with momenta $p_1,\ldots,p_m$ and flavours $f_1,\ldots,f_m$, and an additional $n-m$ colourless particles. The momenta of the incoming and outgoing partons are always considered in the physical region
\begin{align}
    p_i \cdot p_j > 0\,, \quad i\neq j\,, \quad i,j = 1,\ldots,m\,.
\end{align}
The \emph{bare} amplitude admits a perturbative expansion in the strong coupling $\as$ as follows,
\begin{align}
    \mathcal{M} = \left(\frac{\as}{2\pi}\right)^{r}
    \left[\mathcal{M}^{(0)}+
    \frac{\as}{2\pi}\mathcal{M}^{(1)}
    +\left(\frac{\as}{2\pi}\right)^2\mathcal{M}^{(2)}+ \mathcal{O}\left(\as^3\right)
    \right]\,.
    \label{eq:ampl_exp}
\end{align}
where in general $r=s/2$ with $s\in \mathbb{N}$, $\mathcal{M}^{(0)}$ denotes the lowest order contribution to the scattering process\footnote{For our purposes the quantity $\mathcal{M}^{(0)}$ will denote the tree amplitude, though this is not always true. For instance, diphoton production via gluon fusion, $gg\to \gamma\gamma$, is a loop-induced process at leading order.} and $\mathcal{M}^{(k)}$ with $k\geq 1$ denotes the $k$-loop correction. The dependence of the amplitude on the external momenta $p_i$ is not shown explicitly. 

It is often convenient to work with renormalised amplitudes, which are obtained from bare amplitudes by replacing the bare coupling $\as$ with the running coupling $\alpha_{s}(\mu^2)$ evaluated at the renormalisation scale $\mu^2$.
In the $\overline{\textrm{MS}}$ scheme the running coupling can be written as follows,
\edit{factor $S_\e$ on LHS implies that bare amplitude is normalised by factor $S_\e$ i.e. plugging in running coupling we have $\overline{\text{MS}}$-scheme renormalisation, with constants of $4\pi$ and $\gamma_E$ removed.}
\begin{align}
\alpha_{s,0} \,
S_\epsilon= \alpha_s(\mu^2) 
\left[1-\alpha_s(\mu^2)\frac{\beta^\prime_0}{\epsilon} 
+ \alpha_s^2(\mu^2)\left(\frac{\beta^{\prime\,2}_0}{\epsilon^2}- \frac{\beta^\prime_1}{2\epsilon} \right) + \mathcal{O}\left(\alpha_s^3(\mu^2)\right)\right]\,,
\label{eq:QCD_running}
\end{align}
Here, $\mu_0$ denotes the dimensional regularisation scale which maintains a dimensionless coupling in the bare Lagrangian and $S_\epsilon$ is the phase space volume factor in $D=4-2\epsilon$ dimensions given by\footnote{There are several different ways of defining $\overline{\textrm{MS}}$ scheme including the factor $S_\epsilon$ that lead to identical renormalised Green's functions up to terms of $\mathcal{O}(\epsilon)$.},
\begin{align}
S_\epsilon = \text{exp}[\epsilon(\ln{4\pi} - \gamma_E)] \,,
\end{align}
where $\gamma_E = 0.577215666...$ is the Euler-Mascheroni constant.
The factor $S_\epsilon$ gives the difference with the \emph{minimal subtraction} (MS) scheme in which counterterms are pure poles in $\epsilon=0$. 

The $\beta$-function can be written as a series in the strong-coupling $\alpha_s$,
\begin{align}
    \beta^\prime(\alpha_s) = \alpha_s \sum_{n=0}^{\infty}\beta^\prime_n \left(\frac{\alpha_s}{\pi}\right)^{n+1}\,.
\end{align}
The \ac{qcd} beta function has been computed at three loops by Larin and Vermaseren~\cite{Larin:1993tp}, and at four loops by Czakon~\cite{Czakon:2004bu}, and is known to five-loop accuracy~\cite{Herzog:2017vuf}. The first two coefficients of the QCD beta-function read~\cite{Pokorski:1987ed},
\begin{align}
    \beta_0^\prime = \frac{11C_A-4T_FN^\prime_f}{12\pi}\,, \quad \beta_1^\prime = \frac{17C_A^2 - 10C_AT_FN^\prime_f-6C_FT_F N^\prime_f}{24\pi^2}\,,
    \label{eq:QCD_beta}
\end{align}
for $N^\prime_f$ massless quark flavours. Similarly, for \ac{qed} we have
\begin{align}
\alpha_{0} \,
S_\epsilon= \alpha_s(\mu^2) 
\left[1-\alpha(\mu^2)\frac{\beta_0}{\epsilon} 
+ \alpha^2(\mu^2)\left(\frac{\beta^{2}_0}{\epsilon^2}- \frac{\beta_1}{2\epsilon} \right) + \mathcal{O}\left(\alpha^3(\mu^2)\right)\right]\,,
\label{eq:QED_running}
\end{align}
with
\begin{align}
    \beta_0 = -\frac{N_f}{3\pi}\,, \quad \beta_1 = -\frac{N_f}{4\pi^2}\,,
    \label{eq:QED_beta}
\end{align}
for $N_f$ (active) massless lepton flavours.

Thus, we write the perturbative expansion of the renormalised amplitude $\mathcal{M}_\textrm{R}$ in the running coupling $\alpha_s(\mu^2)$ as follows,
\begin{align}
\begin{split}
    \mathcal{M}_\textrm{R} = \left(\frac{\alpha_s(\mu^2)}{2\pi}\right)^{r}\left\{
    \mathcal M^{(0)}_\textrm{R} +  \frac{\alpha_s(\mu^2)}{2\pi} \mathcal{M}^{(1)}_\textrm{R}
    +\left(\frac{\alpha_s(\mu^2)}{2\pi}\right)^2 
    \mathcal{M}^{(2)}_\textrm{R} 
    + \mathcal{O}\left(\alpha_s^3(\mu^2)\right) 
    \right\}\,.
\end{split}
\label{eq:ampl_renorm_QCD}
\end{align}
The renormalised amplitude coefficients $\mathcal M^{(0)}_\textrm{R},\mathcal M^{(1)}_\textrm{R},\ldots$ acquire an explicit dependence on the renormalisation scale $\mu^2$, though it is not shown. As a final remark, we note that the substitution in eq.~\eqref{eq:QCD_running} is valid when the bare amplitude is evaluated in \ac{cdr}. In any other dimensional regularisation scheme, the running coupling acquires an explicit \ac{rs} dependence~\cite{Catani:1996pk,Catani:1998bh}.


Below, it will be convenient to use the formalism introduced in part~\ref{part:real}, in which amplitudes are interpreted as vectors in an abstract colour $+$ spin space. First, let us review the known infared-singular structure of one-loop \ac{qcd} amplitudes~\cite{Giele:1991vf,Kunszt:1994np,Bern:1993mq,Catani:1996jh,Catani:1996vz}.
The renormalised one-loop coefficient amplitude $|\mathcal{M}_\textrm{R}^{(1)}\rangle$ satisfies a factorisation formula as follows,
\begin{align}
|\mathcal{M}_\textrm{R}^{(1)}\rangle= 
\mathbf{I}^{(1)}(\epsilon)
|\mathcal{M}_\textrm{R}^{(0)}\rangle
+|\mathcal{M}_\textrm{R}^{(1)\, \text{fin}}\rangle\,.
\label{eq:1L_Catani}
\end{align}
where $\mathbf{I}^{(1)}$ is an operator on the colour and spin space of the leading order coefficient amplitude $|\mathcal{M}_\textrm{R}^{(0)}\rangle$. Again, we have suppressed the dependence on the renormalisation scale $\mu^2$ and the external momenta. The factorisation in eq.~\eqref{eq:1L_Catani} is \emph{universal} in that the singular structure is entirely contained in the process-independent one-loop insertion operator $\mathbf{I}^{(1)}$. The quantity $|\mathcal{M}_\textrm{R}^{(1)\, \text{fin}}\rangle$ is finite in the limit $\epsilon \to 0$. The operator $\mathbf{I}^{(1)}$ was derived in ref.~\cite{Catani:1996jh} by integrating all real-radiation graphs of the same order in $\alpha_s$ over the one-particle unresolved phase space. It has the explicit form,
\begin{align}
\mathbf I^{(1)}(\epsilon)= 
\frac{1}{2} \frac{e^{-\epsilon \psi(1)}}{\Gamma(1-\epsilon)} \sum_{i=1}^m \frac{1}{\mathbf{T}_i^2}\mathcal{V}_i(\epsilon) \sum_{\substack{i,j=1\\i\neq j}}^m \mathbf{T}_i\cdot \mathbf{T}_j \left(\frac{\mu^2 e^{-i\lambda_{ij}\pi}}{2p_i\cdot p_j}\right)^{\epsilon}\,,
\label{eq:Ioperator_1L}
\end{align}
where a causal $i\epsilon$-prescription is understood and the flavour-dependent singular function $\mathcal{V}_i(\epsilon)$ in is given by,
\begin{align}
    \mathcal{V}_i(\epsilon) = \mathbf{T}_i^2 \frac{1}{\epsilon^2} + \gamma_{f_i} \frac{1}{\epsilon}\,,
\end{align}
with
\begin{align}
    \gamma_q = \frac{3}{2}C_F\,, \quad \gamma_g = \frac{11}{6}C_A - \frac{2}{3}T_F N_f\,.
\end{align}
The colour charge operators $\mathbf{T}_i$ appearing in eq.~\eqref{eq:Ioperator_1L} were defined in eq.~\eqref{eq:colour_operators}, with $\mathbf{T}_i^2=C_F$ if parton $i$ is a quark (or antiquark) and $\mathbf{T}^2_i=C_A$ if it is a gluon. We can use simple crossing symmetry to relate the colour-charge operators for final state and initial state quarks, 
with $(\mathbf{T}_i^c)_{ab}=-t^c_{b_ia_i}$ if parton $i$ is an initial-state quark and $(\mathbf{T}_i^c)_{ab}=t^c_{a_ib_i}$ if parton $i$ is an initial-state antiquark. The factor $e^{-i\lambda_{ij}\pi}$ in eq.~\eqref{eq:Ioperator_1L} is a unitary phase with
\begin{align}
    \lambda_{ij} =
    \begin{cases}
        &1\,, \quad  i\text{ and }j \text{ are both incoming or outgoing}\,, \\
        &0\,, \quad \text{otherwise}\,.
    \end{cases}
\end{align}
The coefficients $\gamma_i$ can be obtained from the $D$-dimensional integration of the \emph{azimuthally averaged} Altarelli-Parisi splitting functions\footnote{The azimuthal average over the $D-2$ transverse components is equivalent to the average over the spin-polarisation of the parent parton, eq.~\eqref{eq:P_spin_average}, only in the case of \ac{cdr} for which the number of external and internal gluons coincide~\cite{Catani:1996pk}. Thus, in general, the azimuthal average takes on an explicit \ac{rs} dependence.}. Using the fact that the coefficient amplitudes are colour singlet states, i.e. they satisfy,
\begin{align}
    \sum_{i=1}^m \mathbf{T}_i |\mathcal{M}\rangle =0\,,
    \label{eq:colour_conservation_catani}
\end{align}
it is easy to see that there are no colour correlations at $\mathcal{O}(1/\epsilon^2)$. Finally, we note that in eq.~\eqref{eq:1L_Catani} terms of $\mathcal{O}(\epsilon)$ have an explicit  \ac{rs}-dependence.

For $m=2$ partons the colour structure in eq.~\eqref{eq:Ioperator_1L} can be simplified using
\begin{align}
    \mathbf{T}_1\cdot \mathbf{T}_2 = \mathbf{T}_2\cdot \mathbf{T}_1 = - \mathbf{T}_1^2 \equiv - \mathbf{T}_2^2\,,
\end{align}
and we obtain 
\begin{align}
\mathbf I^{(1)}_{f_1f_2}(\epsilon)= 
-\mathcal{V}_1(\epsilon) \frac{e^{-\epsilon \psi(1)}}{\Gamma(1-\epsilon)} \left(\frac{\mu^2 e^{-i\lambda_{12}\pi}}{2p_1\cdot p_2}\right)^{\epsilon}\,,
\label{eq:Ioperator_1L_2partons}
\end{align}
where $(f_1,f_2)\in\{(g,g),(q,\bar{q}),(\bar{q},\bar{q}),(q,q)\}$. Clearly, the factorisation is exact in the colour space of the amplitude.

Likewise, the factorisation of two-loop amplitudes is universal, with~\cite{Catani:1998bh}
\begin{align}
|\mathcal{M}_\textrm{R}^{(2)}\rangle= 
\mathbf{I}^{(1)}(\epsilon)
|\mathcal{M}_\textrm{R}^{(1)}\rangle
+\mathbf{I}^{(2)}(\epsilon)
|\mathcal{M}_\textrm{R}^{(0)}\rangle
+|\mathcal{M}_\textrm{R}^{(2)\, \text{fin}}\rangle\,.
\label{eq:2L_Catani_QCD}
\end{align}
Above, the one-loop insertion operator $\mathbf I^{(1)}$ acts on the renormalised one-loop amplitude $|\mathcal{M}_\textrm{R}^{(1)}\rangle$ and contains poles up to $\mathcal{O}(1/\epsilon^4)$. The two-loop insertion operator $\mathbf I^{(2)}$ has the form,
\begin{align}
\begin{split}
\mathbf I^{(2)}(\epsilon)  &= 
- \frac{1}{2} \mathbf I^{(1)}(\epsilon) 
\left( 
\mathbf I^{(1)}(\epsilon) + \frac{4\pi \beta_0 }{\epsilon}
\right) 
+ \frac{e^{\epsilon\psi(1)} \Gamma(1-2\epsilon)}{\Gamma(1-\epsilon)}\left(\frac{2\pi \beta_0 }{\epsilon} + K^\prime \right) \mathbf I^{(1)}(2\epsilon) +\mathbf H^{(2)}(\epsilon) \,,
\end{split}
\label{eq:2L_Catani_operator}
\end{align}
with
\begin{align}
K^\prime = \left(\frac{67}{18}-\frac{\pi^2}{6}\right)C_A-\frac{10}{9}T_FN_f\,.
\end{align}
The process-dependent operator $\mathbf{H}^{(2)}$ contains single and double poles in $\epsilon$~\cite{Catani:1998bh,Aybat:2006mz,Anastasiou:2000kg,Anastasiou:2000ue,Anastasiou:2001sv,Bern:2003ck,Glover:2004si,DeFreitas:2004kmi,Glover:2001af,Bern:2002tk,Garland:2001tf,Garland:2002ak,Bern:2004cz}. The entire \ac{rs}-dependence of the factorisation formula in eq.~\eqref{eq:2L_Catani_QCD} is contained in the two-loop finite remainder $|\mathcal{M}_\textrm{R}^{(2)\, \text{fin}}\rangle$ and terms in  $\mathbf{H}^{(2)}$ of $\mathcal{O}(1/\epsilon)$. Since we always work in \ac{cdr} we will not mention this further.

We denote the universal one- and two-loop insertion coefficients for the process in eq.~\eqref{eq:basic-processes} by $I_{ee\to n\gamma}^{(1)}$ and $I_{ee\to n\gamma}^{(2)}$. The renormalised one-loop annihilation amplitude satisfies the following factorisation formula
\begin{align}
\mathcal{M}_\textrm{R}^{(1)} = 
I^{(1)}_{ee\to n\gamma}(\epsilon)
\mathcal{M}_\textrm{R}^{(0)}
+\mathcal{M}_\textrm{R}^{(1)\, \text{fin}}\,.
\label{eq:1L_Catani_QED}
\end{align}
with \edit{the factor $n{\pi\beta_0}/{\epsilon}$ is probably equivalent to $n H_\gamma^{(1)}$ in analogy to two-loop insertion operator.}
\begin{align}
I^{(1)}_{ee\to n\gamma} = 
-\left( \frac{\mu^2}{-2p_1\cdot p_2} \right)^\epsilon
\frac{e^{-\epsilon \psi(1)}}{\Gamma(1-\epsilon)} 
\left(\frac{1}{\epsilon^2} + \frac{3}{2\epsilon} +n\frac{\pi\beta_0}{\epsilon}\right)\,.
\label{eq:Ioperator_1L_QED}
\end{align}
At two loops, we have
\begin{align}
\mathcal{M}_\textrm{R}^{(2)} = 
I^{(1)}_{ee\to n\gamma}(\epsilon)
\mathcal{M}_\textrm{R}^{(1)}
+I^{(2)}_{ee\to n\gamma}(\epsilon)
\mathcal{M}_\textrm{R}^{(0)}
+\mathcal{M}_\textrm{R}^{(2)\, \text{fin}}\,,
\label{eq:2L_Catani_QED}
\end{align}
\begin{align}
\begin{split}
I_{ee\to n\gamma}^{(2)}(\epsilon)  &= 
- \frac{1}{2} I_{ee\to n\gamma}^{(1)}(\epsilon) 
\left( 
I_{ee\to n\gamma}^{(1)}(\epsilon) + \frac{4\pi \beta_0 }{\epsilon}
\right)  \\
&+ \frac{e^{\epsilon\psi(1)} \Gamma(1-2\epsilon)}{\Gamma(1-\epsilon)}\left(\frac{2\pi \beta_0 }{\epsilon} + K \right) I_{ee\to n\gamma}^{(1)}(2\epsilon) +H_{ee\to n\gamma}^{(2)}(\epsilon) \,,
\end{split}
\label{eq:2L_Catani_QED_operator}
\end{align}
where
\begin{align}
K =- \frac{10}{9} N_f\,.
\end{align}
For the processes under study, the operator $ H_{ee\to n\gamma}^{(2)}$ can be decomposed into~\cite{Anastasiou:2002zn}
\edit{here, operator evaluated in CDR! In general regularisation scheme dependent (at one loop only the finite terms are).}
\begin{align}
H_{ee\to n\gamma}^{(2)} &=
\frac{1}{4\epsilon} \frac{e^{-\epsilon \psi(1)}}{\Gamma(1-\epsilon)} 
\left( \frac{\mu^2}{-2p_1\cdot p_2} \right)^{2\epsilon}
\left(H^{(2)}_{e^+}+H^{(2)}_{e^-} + n H^{(2)}_\gamma \right)\,,
\end{align}
which contains only single poles, where for each external (anti-)quark we have
\begin{align}
\begin{split}
H^{(2)}_q = H^{(2)}_{\bar{q}} &= \left(\frac{\pi^2}{2} -6 \zeta_3 - \frac{3}{8} \right)C_F^2
+\left(\frac{13}{2}\zeta_3 + \frac{245}{216} 
-\frac{23}{48}\pi^2\right)C_A C_F
\\&+ \left( \frac{\pi^2}{12} -\frac{25}{54}\right)T_F N_f^\prime C_F\,, 
\end{split}
\end{align}
and for each external photon,
\begin{align}
H^{(2)}_\gamma &= \frac{20}{27}N_f^2 + N_f\,.
\end{align}
where $H^{(2)}_{e^+} = H^{(2)}_{e^-} \equiv H^{(2)}_e$. 

It will be useful to consider a version of eq.~\eqref{eq:2L_Catani_QED} valid for the bare two-loop amplitude $\mathcal{M}^{(2)}$, obtained by inverting eqs.~\eqref{eq:QED_running}, \eqref{eq:M1renorm} and~\eqref{eq:M2renorm} in terms of bare parameters. The running coupling $\alpha(\mu^2)$ as a function of $\alpha_0$ becomes,
\begin{align}
    \alpha(\mu^2) = \alpha_0 S_\e  +  \alpha_0^2 S_\e^2 \frac{\beta_0}{\e} +  \alpha_0^3 S_\e^3 \left(\frac{\beta_0^2}{\e^2} + \frac{\beta_1}{2\e}\right) + \mathcal{O}(\alpha_0^4)\,.
\end{align}
The bare one-loop amplitude $\cM^{(1)}$ factorises as
\edit{overall factor $S_\e$ is equivalent to $(4\pi)^\epsilon e^{\epsilon\psi(1)}$ normalisation that we use for our amplitudes. So we should remove this factor below to be consistent (and use $S_\epsilon$ everywhere). Either leave it there or remove it and write expansion in eq.~\eqref{eq:M_series} in terms of $\alpha_{s,0} S_\epsilon$. Then it's consistent, also with definition of Catani operators and running coupling}
\begin{align}
\begin{split}
        \mathcal{M}^{(1)} &= I^{(1)\,\text{bare}}_{ee\to n\gamma} \cM^{(0)} +\mathcal{M}^{(1)\,\text{fin}} 
        \\&=
        S_\e\left(I^{(1)}_{ee\to n\gamma} + n\frac{\pi\beta_0}{\e} \right) \mathcal{M}^{(0)}+\mathcal{M}^{(1)\,\text{fin}}\,,
\end{split}
\label{eq:1L_Catani_bare}
\end{align}
\edit{problem: if you expand $(I^{(1)}_{ee\to n\gamma} + n\frac{\pi\beta_0}{\e})^2$ then you will not get something independent of $n$. So strictly speaking the discussion below is wrong. Just set $n\to 0$ everywhere to get the bare operators}

where the second equality was obtained by substituting eq.~\eqref{eq:M1renorm} into eq.~\eqref{eq:1L_Catani}. This defines the universal, ``bare" one-loop insertion operator as follows,
\begin{align}
I^{(1)\,\text{bare}}_{ee\to n\gamma} = 
-\left( \frac{4\pi \mu^2}{-2p_1\cdot p_2} \right)^\e
\frac{1}{\Gamma(1-\e)} 
\left(\frac{1}{\e^2} + \frac{3}{2\e} \right)\,.
\label{eq:Ioperator_1L_bare}
\end{align}

Next, we plug in eqs.~\eqref{eq:M1renorm} and~\eqref{eq:M2renorm} into the two-loop factorisation formula, eq.~\eqref{eq:2L_Catani_QED}, and solve for the bare two-loop amplitude $\mathcal{M}^{(2)}$,
\edit{as above all factors of $S_\e$ should be removed to stay consistent}
\begin{align}
\begin{split}
    \mathcal{M}^{(2)} &= 
    \left(I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e)
    + S_\e\frac{2\pi\beta_0}{\e}\right) \mathcal{M}^{(1)} 
    +
    S_\e^2
    I_{ee\to n\gamma}^{(2)\,\text{bare}}(\e)
    \mathcal{M}^{(0)}\,.
\end{split}
\end{align}
\edit{where $I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e)$ and $I_{ee\to n\gamma}^{(2)\,\text{bare}}(\e)$ are obtained by setting $n=0$}
Therefore, we write the factorisation formula for the bare two-loop amplitude as
\begin{align}
\mathcal{M}^{(2)}&= 
\left( I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e) + S_\e\frac{2\pi\beta_0}{\e}\right)\mathcal{M}^{(1)}
+ I_{ee\to n\gamma}^{(2)\,\text{bare}}(\e) 
 \mathcal{M}^{(0)}
+ \mathcal{M}^{(2)\,\text{fin.}}\,.
\label{eq:M2_catani_bare}
\end{align}
The corresponding two-loop insertion coefficient is given by \edit{wrong}
\begin{align}
\begin{split}
I_{ee\to n\gamma}^{(2)\,\text{bare}}(\e)  &= 
- \frac{1}{2} I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e) 
\left( 
I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e) + S_\e \frac{4\pi \beta_0 }{\e}
\right)  \\
&+ \frac{e^{\e\psi(1)} \Gamma(1-2\e)}{\Gamma(1-\e)}\left(\frac{2\pi \beta_0 }{\e} + K \right) I_{ee\to n\gamma}^{(1)\,\text{bare}}(2\e) + H_{ee\to n\gamma}^{(2)\,\text{bare}}(\e) \,,
\end{split}
\label{eq:2L_Catani_bare}
\end{align}
where \edit{this is correct}
\begin{align}
    H_{ee\to n\gamma}^{(2)\,\text{bare}}(\e) = 
    \frac{1}{4\e}\frac{e^{\e \psi(1)}}{\Gamma(1-\e)} \left( \frac{4\pi\mu^2}{-2p_1\cdot p_2} \right)^{2\e}
    (H^{(2)}_{e^+} + H^{(2)}_{e^-})\,.
\end{align}
Combining eqs.~\eqref{eq:1L_Catani_bare} and~\eqref{eq:M2_catani_bare} the singularity structure can be re-organised as follows,
\begin{align}
\begin{split}
\mathcal{M}^{(2)}&= 
\left[I_{ee\to n\gamma}^{(2)\,\text{bare}}(\epsilon)+
I^{(1)\,\text{bare}}_{ee\to n\gamma}(\epsilon)\left(I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e) + S_\e\frac{2\pi\beta_0}{\e}\right)\right]\cM^{(0)}
\\&\quad+\left(I_{ee\to n\gamma}^{(1)\,\text{bare}}(\e) + S_\e\frac{2\pi\beta_0}{\e}\right)\mathcal{M}^{(1)\,\text{fin}}
+ \mathcal{M}^{(2)\,\text{fin.}}\,.
\end{split}
\label{eq:M2_catani_bare_v2}
\end{align}





==> ward_3L.tex <==
\section{Three-loop Ward identities}
\label{sec:ward_3L}

\subsection{Three-loop two- and three-point Green's functions}
\label{sec:Greens_3L}

